Graph Analytics using the Vertica Relational Database

Graph analytics is becoming increasingly popular, with a deluge of new systems for graph analytics having been proposed in the past few years. These systems often start from the assumption that a new storage or query processing system is needed, in spite of graph data being often collected and stored in a relational database in the first place. In this paper, we study Vertica relational database as a platform for graph analytics. We show that vertex-centric graph analysis can be translated to SQL queries, typically involving table scans and joins, and that modern column-oriented databases are very well suited to running such queries. Specifically, we present an experimental evaluation of the Vertica relational database system on a variety of graph analytics, including iterative analysis, a combination of graph and relational analyses, and more complex 1- hop neighborhood graph analytics, showing that it is competitive to two popular vertex-centric graph analytics systems, namely Giraph and GraphLab.

==> 6-discussion.tex <==
\section{Lessons Learned}
\label{section:lessons}

Below we describe the key takeaways from our analysis and evaluation in this paper.

\noindent\textbf{Graph analytics can be expressed and tuned in RDBMSs.} Relational databases are general purpose data processing systems and graph operations can be expressed as relational operators in a relational database. Furthermore, relational databases can be effectively tuned to offer good performance on graph queries, yielding performance that is competitve with dedicated graph stores.
\noindent\textbf{Column-oriented databases excels at graph analytics.} We showed that the analytic-optimized relational databases like Vertica can have significantly better performance than popular graph processing systems (specifically, Giraph) on a variety of graph analytics. 
This is because these queries typically involves full scans, joins, and aggregates over large tables, for which Vertica is heavily optimized.
These optimizations include efficient physical data representation (columnar layout, compression, sorting, segmentation), pipelined query execution, and an optimizer to automatically pick the best physical plan at runtime.
This is in contrast to Giraph which has a static query execution pipeline and blocks the query execution before running the vertex functions.


\noindent\textbf{Some graph queries are difficult to express in vertex-centric graph systems.} We showed that the vertex-centric programming model is a poor fit for several complex graph analyses. In particular, it is very difficult to program and run graph analysis involving 1-hop neighborhoods on vertex-centric systems -- indeed, we could not get Giraph to execute many such analyses on even modest-sized graphs. This is because the scope of vertex-centric computations is restricted to a vertex and its immediate neighbors. In contrast, relational databases do not have such limitations and are able to efficiently execute 1-hop neighborhood computations.

\noindent\textbf{The RDBMS advantage: Graph + Relational Analysis.} Apart from outperforming graph processing systems on graph analysis, the real advantage of relational databases is the ability to combine graph analysis with relational analysis. This is because graph analysis is typically accompanied by relational analysis, either as a preparatory step or as a final reporting step. Such relational analysis is either impossible or highly inefficient in graph processing systems, while is natural to express in relational databases.

\noindent\textbf{RDBMSs are a box full of goodies.} Relational databases come with many features that are not present (yet) in the next generation of graph processing systems. 
These include update handling, transactions, checkpointing and recovery, fault tolerance, durability, integrity constraints, type checking, ACID etc.
Current-generation graph processing systems simply do not come with this rich set of features.
One might think of stitching multiple systems together and coordinating between them to achieve these features, e.g.~using HBase for transactions and Giraph for analytics, but then we have the additional overhead of stitching these systems together. 
Of course, with time, graph-engines may evolve these features, but our results suggest that these graph systems should be layered on RDBMS, not built outside of them, which would enable them to inherit these features for free without giving up performance.
Furthermore, in many scenarios, the raw data for the graphs is maintained in a relational database in the first place. In such situations, it would make sense to be able to perform graph analytics within the same system.

\noindent\textbf{Programming Model.}  One argument against using relational databases is that some users prefer the vertex-centric programming model, because writing graph analytics in SQL requries reasoning in terms of tables rather than nodes and edges.  For users who feel this way, we are currently implementing a vertex-centric layer on top of a SQL engine, providing the naturalness of the vertex-centric model with the performance and features of relational engines.


